Marked Personas: Using Natural Language Prompts to Measure Stereotypes in Language Models

To recognize and mitigate harms from large language models (LLMs), we need to understand the prevalence and nuances of stereotypes in LLM outputs. Toward this end, we present Marked Personas, a prompt-based method to measure stereotypes in LLMs for intersectional demographic groups without any lexicon or data labeling. Grounded in the sociolinguistic concept of markedness (which characterizes explicitly linguistically marked categories versus unmarked defaults), our proposed method is twofold: 1) prompting an LLM to generate personas, i.e., natural language descriptions, of the target demographic group alongside personas of unmarked, default groups; 2) identifying the words that significantly distinguish personas of the target group from corresponding unmarked ones. We find that the portrayals generated by GPT-3.5 and GPT-4 contain higher rates of racial stereotypes than human-written portrayals using the same prompts. The words distinguishing personas of marked (non-white, non-male) groups reflect patterns of othering and exoticizing these demographics. An intersectional lens further reveals tropes that dominate portrayals of marginalized groups, such as tropicalism and the hypersexualization of minoritized women. These representational harms have concerning implications for downstream applications like story generation.

==> both.tex <==

% \begin{table*}[ht]
%     \begin{tabular}{l|p{0.85\linewidth}}
%     \textbf{Group}&\textbf{Significant Words}\\\hline        
% Black&
% black strength curly beautiful
% \\
% Asian&
% asian almondshaped dark petite smooth traditional black chinese
% \\
% ME&
% middleeastern traditional dark headscarf thick hijab olive clothing head wear religious abaya long beard faith middle scarf
% \\
% Latine&
% latina latino latin spanish dark vibrant heritage music proud culture passionate dancing
% \\
% White&
% blue blonde white fair light green
% \\
% woman&
% her woman she women latina delicate long beautiful petite beauty grace figure herself hijab natural colorful curves intricate jewelry falls
% \\
% man&
% his he man beard short latino men him neatly build jawline medium trimmed shirt broad muscular sports a jeans tall himself athletic physique crisp
% \\
% Black W&
% her beautiful strength resilience
% \\
% Asian W&
% her asian petite almondshaped smooth
% \\
% ME W&
% her hijab middleeastern abaya modest long colorful
% \\
% Latina W&
% her latina vibrant
% \\

%     \end{tabular}
%     \caption{\textbf{Top words for each group (ChatGPT).} TODO caption}
%     \label{tab:topwords_chat}
% \end{table*}

==> d.tex <==
\textcolor{blue}{\textbf{middleeastern}, \textbf{\textit{traditional}}, \textbf{dark}, \textbf{\textit{headscarf, thick, hijab,}} \textit{olive}, clothing, head, wear, religious,
abaya, long, \textit{beard}, faith, middle, scarf}, keffiyeh, \textit{olivetoned}, \textbf{his}, thobe, \textit{flowing}, garment, attire, modest, eyebrows, bustling, intricate, region, abaya, anklelength, her,  \textbf{strong}, \textbf{deep}, loosefitting, \textit{adorned}, draped, thawb, embroidery, faith, middle, \textbf{rich}, prominent, arabic, desert, modesty, agal, the, scarf, marketplace, market, garments, worn, covered, \textcolor{gray}{(wisdom)}

==> extra_intro.tex <==

Language models (LMs) excel at instruction-based tasks, such as generating realistic stories without any fine-tuning \citep{liang2022holistic,ouyang2022training}. 
% While an LM's outputs may contain differences when prompted with different text, these differences ought not to be harmful to marginalized people. 
They should not contain \textit{stereotypes}: traits that have been documented to be broadly associated with a demographic group in ways that reify existing social hierarchies \citep{
deaux1993gender, 
heilman2001description, caliskan2017semantics,blodgett2021stereotyping,weidinger2021ethical}.
